Defurnishing with X-Ray Vision: Joint Removal of Furniture from Panoramas and Mesh

We present a pipeline for generating defurnished replicas of indoor spaces represented as textured meshes and corresponding multi-view panoramic images. To achieve this, we first segment and remove furniture from the mesh representation, extend planes, and fill holes, obtaining a simplified defurnished mesh (SDM). This SDM acts as an ``X-ray'' of the scene's underlying structure, guiding the defurnishing process. We extract Canny edges from depth and normal images rendered from the SDM. We then use these as a guide to remove the furniture from panorama images via ControlNet inpainting. This control signal ensures the availability of global geometric information that may be hidden from a particular panoramic view by the furniture being removed. The inpainted panoramas are used to texture the mesh. We show that our approach produces higher quality assets than methods that rely on neural radiance fields, which tend to produce blurry low-resolution images, or RGB-D inpainting, which is highly susceptible to hallucinations.

==> TODO.tex <==
%- improve result images for teaser (run more spaces)
%- pipeline image
%- pipeline image: cut top and bottom poles from panos
%- pipeline image: remove red circle from untextured SDM
%- hole filling image: update to snapshots without trackball and with transparent background; zoom in to issues/ show other viewpoints
%- cite CMU folks that keep on citing us
%- cite Multi-HexPlanes
%- find another competitive method that is not hard to set up (e.g. check PixelSynth, CompNVS)
%- talk about SDS either in related work or in the radiance field section of comparisons
%- get mesh from the Nerfiller checkpoint on the ScanNet data
%- images in ScanNet data figure: crop to content in GIMP and export as smaller files
%- figure 2 should be where figure 5 is right now (results)
% - POLES! REMOVE THEM! :de:
%- hole filling figure: overlays and boxes
%- sneak mesh metrics on synthetic data into Nerfiller text

Supplementary:
%- Instruct-NeRF2NeRF and Instruct-GS2GS example on Matterport3D, modify main text accordingly
%- Show Nerfiller meshes and images on ScanNet
%- Explain how we run Nerfiller, especially small vs big spaces
%- Perspective images corresponding to the panos
- Info on synthetic data experiment
- Add a sentence to briefly explain each figure in the first section


% TODO(03/03)
%- SuperResolution section (Gregor? we could also leave it as is)

%- Failures - 3 x horizonal -> move input images to supplementary.
%- Hole filling - copy to supplementary and leave top row 


% - Change bottom figure of Figure 4 Ablations -> tis ugly

